Identification and Bounding of Central Moments of Causal Effects Using Marginal Moments Information

Evaluating the causal effect of a treatment on an outcome is a central objective in causal inference. While the average causal effect summarizes the mean impact of treatment, the central moments of the individual causal effect (ICE) characterize the shape of the ICE distribution, thereby revealing the extent and structure of treatment effect heterogeneity across individuals. This paper investigates the identification and bounding of the central moments of the ICE using only the marginal central moments of each potential outcome (PO). Compared with existing approaches that require knowledge of the full marginal distributions of the POs, marginal moment information is often substantially easier to obtain in empirical applications. Finally, we illustrate the practical relevance of our results through two empirical case studies.

==> 4-8_Taking_intersection.tex <==



%We briefly discuss the case where we have $(\overline{\sigma}_1^{(k)},\overline{\sigma}_0^{(k)})$ for at least two distinct $k$.


We can derive tight bounds of $\overline{\mu}^{(m)}$ ($m=2,3,4$) 
using a combination of ($\overline{\sigma}_1^{(2)}$,$\overline{\sigma}_0^{(2)}$),
($\overline{\sigma}_1^{(3)}$,$\overline{\sigma}_0^{(3)}$),
and ($\overline{\sigma}_1^{(4)}$,$\overline{\sigma}_0^{(4)})$, by combining theorems in this paper.
%We briefly discuss how to combine information when more than one of
%$(\overline{\sigma}_1^{(2)},\overline{\sigma}_0^{(2)})$,
%$(\overline{\sigma}_1^{(3)},\overline{\sigma}_0^{(3)})$,
%and $(\overline{\sigma}_1^{(4)},\overline{\sigma}_0^{(4)})$ is available.
%In such cases, we can potentially tighten the bound on $\overline{\mu}^{(m)}$ for $m\in\{2,3,4\}$ by intersecting the bounds obtained from each available moment order.
\begin{proposition}
Let $T\subset\{2,3,4\}$ be a set of available moment orders of $(\overline{\sigma}_1^{(k)},\overline{\sigma}_0^{(k)})$.
For each $m\in\{2,3,4\}$ and $k\in T$, letting $[L_{m,k},U_{m,k}]$ be the bound on $\overline{\mu}^{(m)}$ derived from each $(\overline{\sigma}_1^{(k)},\overline{\sigma}_0^{(k)})$,
%Then the intersection is also a bound on $\overline{\mu}^{(m)}$. In other words, 
we have
\begin{equation}
\overline{\mu}^{(m)} \in \bigcap_{k\in T}[L_{m,k},U_{m,k}]
= \big[\max_{k\in T} L_{m,k},\min_{k\in T} U_{m,k}\big].
\end{equation}
\end{proposition}
%This bound is never wider than any single bound in the intersection.
%It is strictly tighter whenever at least one endpoint improves.

%%%%%%%%%%%
\iffalse
For example, assuming $(\overline{\sigma}_1^{(2)},\overline{\sigma}_0^{(2)})$ and $(\overline{\sigma}_1^{(4)},\overline{\sigma}_0^{(4)})$ are available, we have
\begin{equation}
\begin{aligned}
    \overline{\mu}^{(4)}\in & \Big[ \min\Big\{\big(\sqrt{\overline{\sigma}_1^{(2)}}-\sqrt{\overline{\sigma}_0^{(2)}}\big)^4,  \big(\sqrt[4]{\overline{\sigma}_1^{(4)}}-\sqrt{\overline{\sigma}_0^{(4)}}\big)^4 \Big\}, \\
    &  \qquad \qquad  \big(\sqrt[4]{\overline{\sigma}_1^{(4)}}+\sqrt{\overline{\sigma}_0^{(4)}}\big)^4\Big].
\end{aligned}
\end{equation}
\fi
%%%%%%%%%%

%%%%%%%%
\iffalse
\begin{equation}
\begin{aligned}
    \overline{\mu}^{(4)} & \in \Big[\Big(\sqrt{\overline{\sigma}_1^{(2)}}-\sqrt{\overline{\sigma}_0^{(2)}}\Big)^4,\infty \Big) \\
    %\cap [0,\infty) \\
    & \qquad \cap \Big[\Big(\sqrt[4]{\overline{\sigma}_1^{(4)}}-\sqrt{\overline{\sigma}_0^{(4)}}\Big)^4,\Big(\sqrt[4]{\overline{\sigma}_1^{(4)}}+\sqrt{\overline{\sigma}_0^{(4)}}\Big)^4\Big]\\
    & =\Big[\max\Big\{\Big(\sqrt{\overline{\sigma}_1^{(2)}}-\sqrt{\overline{\sigma}_0^{(2)}}\Big)^4,  \Big(\sqrt[4]{\overline{\sigma}_1^{(4)}}-\sqrt{\overline{\sigma}_0^{(4)}}\Big)^4 \Big\}, \\
    &\qquad \Big(\sqrt[4]{\overline{\sigma}_1^{(4)}}+\sqrt{\overline{\sigma}_0^{(4)}}\Big)^4\Big]
\end{aligned}
\end{equation}
\fi
%%%%%%%%%%%%%%
%%%%%%%%%%%%%
\iffalse
\yuta{[Provide simple example]}

On the other hand, if one bound is already tighter than another, then taking the intersection does not yield any further improvement.
Specifically, if $[L_{m,k_1},U_{m,k_1}] \subset [L_{m,k_2},U_{m,k_2}]$ for some $k_1,k_2\in T$, then
$[L_{m,k_1},U_{m,k_1}] \cap [L_{m,k_2},U_{m,k_2}]= [L_{m,k_1},U_{m,k_1}]$.

For example, since $\overline{\sigma}_x^{(2)}\leq \sqrt{\overline{\sigma}_x^{(4)}}$ holds by the Cauchy-Schwarz inequality, if $(\overline{\sigma}_1^{(2)},\overline{\sigma}_0^{(2)})$ and $(\overline{\sigma}_1^{(4)},\overline{\sigma}_0^{(4)})$ are available, the bound obtained in this way is the same as the one in Theorem \ref{thm:bound_of_var}.

\fi
%%%%%%%%%%%%%%

Explicitly, we have the following bounds by combinations of $(\overline{\sigma}_1^{(k)},\overline{\sigma}_0^{(k)})$:

(1) When ($\overline{\sigma}_1^{(2)}$,\,$\overline{\sigma}_0^{(2)}$) and 
($\overline{\sigma}_1^{(3)}$,\,$\overline{\sigma}_0^{(3)}$) are available, we have
%\begin{equation}
\begin{align}
    \Big(\sqrt{\overline{\sigma}^{(2)}_1}-\sqrt{\overline{\sigma}^{(2)}_0}\Big)^2\leq \overline{\mu}^{(2)}
    &\leq \Big(\sqrt{\overline{\sigma}^{(2)}_1}+\sqrt{\overline{\sigma}^{(2)}_0}\Big)^2, \\
    -\infty <\overline{\mu}^{(3)}&<\infty, \\
    \Big(\sqrt{\overline{\sigma}_1^{(2)}}-\sqrt{\overline{\sigma}_0^{(2)}}\Big)^4
\leq \overline{\mu}^{(4)} &< \infty.    
\end{align}
%\end{equation}

(2) When ($\overline{\sigma}_1^{(2)}$,\,$\overline{\sigma}_0^{(2)}$) and ($\overline{\sigma}_1^{(4)}$,\,$\overline{\sigma}_0^{(4)}$) are available, we have
%\begin{equation}
\begin{align}
    \Big(\sqrt{\overline{\sigma}^{(2)}_1}-\sqrt{\overline{\sigma}^{(2)}_0}\Big)^2 & \leq \overline{\mu}^{(2)}
    \leq \Big(\sqrt{\overline{\sigma}^{(2)}_1}+\sqrt{\overline{\sigma}^{(2)}_0}\Big)^2, \\
    -\frac{\sqrt{2}}{\sqrt[4]{27}}\Bigl(\sqrt[4]{\overline{\sigma}_1^{(4)}}+\sqrt[4]{\overline{\sigma}_0^{(4)}}\Bigr)^3  &\leq \overline{\mu}^{(3)} \nonumber\\
    &\leq \frac{\sqrt{2}}{\sqrt[4]{27}}\Bigl(\sqrt[4]{\overline{\sigma}_1^{(4)}}+\sqrt[4]{\overline{\sigma}_0^{(4)}}\Bigr)^3, \\
    \max\Big\{
    \big(\sqrt{\overline{\sigma}_1^{(2)}}-\sqrt{\overline{\sigma}_0^{(2)}}\big)^4, &  \big(\sqrt[4]{\overline{\sigma}_1^{(4)}}-\sqrt{\overline{\sigma}_0^{(4)}}\big)^4 
    \Big\} \nonumber\\
    & \leq \overline{\mu}^{(4)} \leq \big(\sqrt[4]{\overline{\sigma}_1^{(4)}}+\sqrt{\overline{\sigma}_0^{(4)}}\big)^4.  
\end{align}
%\end{equation}

(3) When ($\overline{\sigma}_1^{(3)}$,\,$\overline{\sigma}_0^{(3)}$) and ($\overline{\sigma}_1^{(4)}$,\,$\overline{\sigma}_0^{(4)}$) are available, we have
%\begin{equation}
\begin{align}
    0 & \leq \overline{\mu}^{(2)} \leq \Big(\sqrt[4]{\overline{\sigma}_1^{(4)}}+\sqrt[4]{\overline{\sigma}_0^{(4)}}\Big)^2, \\
    -\frac{\sqrt{2}}{\sqrt[4]{27}}\Bigl(\sqrt[4]{\overline{\sigma}_1^{(4)}}+\sqrt[4]{\overline{\sigma}_0^{(4)}}\Bigr)^3  &\leq \overline{\mu}^{(3)}  \nonumber\\
    &\leq \frac{\sqrt{2}}{\sqrt[4]{27}}\Bigl(\sqrt[4]{\overline{\sigma}_1^{(4)}}+\sqrt[4]{\overline{\sigma}_0^{(4)}}\Bigr)^3,\\
    \Big(\sqrt[4]{\overline{\sigma}^{(4)}_1}-\sqrt[4]{\overline{\sigma}^{(4)}_0}\Big)^4 \nonumber
    &\leq
    \overline{\mu}^{(4)}
    \leq
    \Big(\sqrt[4]{\overline{\sigma}^{(4)}_1}+\sqrt[4]{\overline{\sigma}^{(4)}_0}\Big)^4.    
\end{align}
%\end{equation}

(4) When ($\overline{\sigma}_1^{(2)}$,\,$\overline{\sigma}_0^{(2)}$),
($\overline{\sigma}_1^{(3)}$,\,$\overline{\sigma}_0^{(3)}$),
and ($\overline{\sigma}_1^{(4)}$,\,$\overline{\sigma}_0^{(4)}$) are available, we have
%\begin{equation}
\begin{align}
\label{eq:bound_of_var_with_234}
    \Big(\sqrt{\overline{\sigma}^{(2)}_1}-\sqrt{\overline{\sigma}^{(2)}_0}\Big)^2 & \leq \overline{\mu}^{(2)}
    \leq \Big(\sqrt{\overline{\sigma}^{(2)}_1}+\sqrt{\overline{\sigma}^{(2)}_0}\Big)^2, \\
    \label{eq:bound_of_mu3_with_234}
    -\frac{\sqrt{2}}{\sqrt[4]{27}}\Bigl(\sqrt[4]{\overline{\sigma}_1^{(4)}}+\sqrt[4]{\overline{\sigma}_0^{(4)}}\Bigr)^3  &\leq \overline{\mu}^{(3)}  \nonumber\\
    &\leq \frac{\sqrt{2}}{\sqrt[4]{27}}\Big(\sqrt[4]{\overline{\sigma}_1^{(4)}}+\sqrt[4]{\overline{\sigma}_0^{(4)}}\Big)^3, \\
    \label{eq:bound_of_mu4_with_234}
    \max\Big\{
    \big(\sqrt{\overline{\sigma}_1^{(2)}}-\sqrt{\overline{\sigma}_0^{(2)}}\big)^4, &  \big(\sqrt[4]{\overline{\sigma}_1^{(4)}}-\sqrt{\overline{\sigma}_0^{(4)}}\big)^4 
    \Big\}  \nonumber\\
    & \leq \overline{\mu}^{(4)} \leq \big(\sqrt[4]{\overline{\sigma}_1^{(4)}}+\sqrt{\overline{\sigma}_0^{(4)}}\big)^4.  
\end{align}
%\end{equation}


\jin{I don't like Proposition 2 or how the results are organized in Eqs. (24)-(35) - difficult to understand the results. To me, it's much better to write results separately for each $\overline{\mu}^{(m)}$ ($m=2,3,4$), that is, for each $\overline{\mu}^{(m)}$, state what bounds we have under what given inputs.}
\naoya{[We obtained tighter bounds for those cases, but these are a little bit complicated and most of them are not moment-sharp or $\varepsilon$-moment-sharp. To obtain ($\varepsilon$-)moment-sharp bound seems to be quite challenging. This is a reason we hesitated to (and did not) include those them here, and left as a future work. But we will reconsider the construction of this section.]}\jin{You could make each subsection focus on an individual $\overline{\mu}^{(m)}$, with different theorems for different possible inputs.}

{\bf Remark on bounding skewness and kurtosis.}
To obtain bounds on skewness of ICE $\overline{\mu}^{(3)} / \{\overline{\mu}^{(2)}\}^{3/2}$ and kurtosis  of ICE $\overline{\mu}^{(4)} / \{\overline{\mu}^{(2)}\}^{2}$, we first compute bounds on $\overline{\mu}^{(k)}$ $(k=2,3,4)$ from the results in this section. 
Then, the upper bound on skewness is given by the ratio of the upper bound of $\overline{\mu}^{(3)}$ to the lower bound of $\overline{\mu}^{(2)}$ raised to the power $3/2$, and the lower bound is the negative of this value. 
The upper (resp. lower) bound on kurtosis is given by the ratio of the upper (resp. lower) bound of $\overline{\mu}^{(4)}$ to the square of the lower (resp. upper) bound of $\overline{\mu}^{(2)}$.
They are not moment-sharp or $\varepsilon$-moment-sharp.

\jin{Think carefully how to better organize the results in Section 5. It's quite messy right now. Perhaps first focus on the individual cases of $\overline{\mu}^{(m)}$ ($m=2,3,4$) under various availability situations of $\overline{\sigma}^{(m)}$ ($m=2,3,4$), with the motivation that we are often interested in variance, skewness, and kurtosis and $\overline{\sigma}^{(m)}$ ($m=2,3,4$) are most likely available in practice. Then have a separate section on $\overline{\mu}^{(m)}$ for arbitrary old/even $m$ that is of more theoretical interest. Extend Theorems 4 and 5, to investigate what bounds can be obtained under what kind of combinations of inputs from $\{\overline{\sigma}^{(m)}\}$, if possible.  }
\naoya{[Theorem 5 can be extended to the case where $\overline{\sigma}_x^{(k)}$ are known for all $k\leq m$ (with condition). The bound of skewness or kurtosis tend to depend on the bound of variance, and they may take quite large values. We willreconsider them.]}


%%%%%%%%%
\iffalse
In our results, the bounds are nested for $m=2$ and $m=3$.
More precisely, the intervals obtained from different moment orders satisfy
\footnote{
We have $[L_{2,4},U_{2,4}] \subset [L_{2,2},U_{2,2}]$ since $\overline{\sigma}_x^{(2)}\leq \sqrt{\overline{\sigma}_x^{(4)}}$ holds by the Cauchy-Schwarz inequality.
}
\begin{equation}
\begin{aligned}
[L_{2,3},U_{2,3}] & \subset [L_{2,4},U_{2,4}] \subset [L_{2,2},U_{2,2}],\\
[L_{3,2},U_{3,2}] & = [L_{3,3},U_{3,3}] \subset [L_{3,4},U_{3,4}].
\end{aligned}
\end{equation}
Therefore, for $m=2$ and $m=3$, intersecting multiple bounds only amounts to using the tightest bound among those available.

In contrast, for $m=4$, the bounds derived from $k=2$ and $k=4$ are not comparable in general.
Hence, their intersection can be strictly tighter than either bound alone, as illustrated by the example above.
\fi
%%%%%%%%%%



==> mu2_app7_2.tex <==
% Created by tikzDevice version 0.12.6 on 2026-02-11 20:57:07
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1.3pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (238.49,173.45);
\begin{scope}
\path[clip] ( 49.20, 61.20) rectangle (213.29,124.25);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] ( 55.28,121.91) --
	( 55.53,121.57) --
	( 55.78,121.23) --
	( 56.04,120.90) --
	( 56.29,120.56) --
	( 56.55,120.22) --
	( 56.80,119.89) --
	( 57.05,119.56) --
	( 57.31,119.22) --
	( 57.56,118.89) --
	( 57.81,118.56) --
	( 58.07,118.24) --
	( 58.32,117.91) --
	( 58.57,117.58) --
	( 58.83,117.26) --
	( 59.08,116.93) --
	( 59.34,116.61) --
	( 59.59,116.29) --
	( 59.84,115.97) --
	( 60.10,115.65) --
	( 60.35,115.33) --
	( 60.60,115.01) --
	( 60.86,114.69) --
	( 61.11,114.38) --
	( 61.37,114.06) --
	( 61.62,113.75) --
	( 61.87,113.44) --
	( 62.13,113.13) --
	( 62.38,112.82) --
	( 62.63,112.51) --
	( 62.89,112.20) --
	( 63.14,111.89) --
	( 63.39,111.59) --
	( 63.65,111.29) --
	( 63.90,110.98) --
	( 64.16,110.68) --
	( 64.41,110.38) --
	( 64.66,110.08) --
	( 64.92,109.78) --
	( 65.17,109.48) --
	( 65.42,109.19) --
	( 65.68,108.89) --
	( 65.93,108.60) --
	( 66.18,108.30) --
	( 66.44,108.01) --
	( 66.69,107.72) --
	( 66.95,107.43) --
	( 67.20,107.14) --
	( 67.45,106.85) --
	( 67.71,106.57) --
	( 67.96,106.28) --
	( 68.21,106.00) --
	( 68.47,105.72) --
	( 68.72,105.43) --
	( 68.97,105.15) --
	( 69.23,104.87) --
	( 69.48,104.59) --
	( 69.74,104.32) --
	( 69.99,104.04) --
	( 70.24,103.76) --
	( 70.50,103.49) --
	( 70.75,103.22) --
	( 71.00,102.94) --
	( 71.26,102.67) --
	( 71.51,102.40) --
	( 71.76,102.13) --
	( 72.02,101.87) --
	( 72.27,101.60) --
	( 72.53,101.33) --
	( 72.78,101.07) --
	( 73.03,100.81) --
	( 73.29,100.54) --
	( 73.54,100.28) --
	( 73.79,100.02) --
	( 74.05, 99.76) --
	( 74.30, 99.51) --
	( 74.55, 99.25) --
	( 74.81, 98.99) --
	( 75.06, 98.74) --
	( 75.32, 98.49) --
	( 75.57, 98.23) --
	( 75.82, 97.98) --
	( 76.08, 97.73) --
	( 76.33, 97.48) --
	( 76.58, 97.24) --
	( 76.84, 96.99) --
	( 77.09, 96.74) --
	( 77.34, 96.50) --
	( 77.60, 96.26) --
	( 77.85, 96.01) --
	( 78.11, 95.77) --
	( 78.36, 95.53) --
	( 78.61, 95.29) --
	( 78.87, 95.05) --
	( 79.12, 94.82) --
	( 79.37, 94.58) --
	( 79.63, 94.35) --
	( 79.88, 94.11) --
	( 80.14, 93.88) --
	( 80.39, 93.65) --
	( 80.64, 93.42) --
	( 80.90, 93.19) --
	( 81.15, 92.96) --
	( 81.40, 92.73) --
	( 81.66, 92.51) --
	( 81.91, 92.28) --
	( 82.16, 92.06) --
	( 82.42, 91.83) --
	( 82.67, 91.61) --
	( 82.93, 91.39) --
	( 83.18, 91.17) --
	( 83.43, 90.95) --
	( 83.69, 90.74) --
	( 83.94, 90.52) --
	( 84.19, 90.30) --
	( 84.45, 90.09) --
	( 84.70, 89.88) --
	( 84.95, 89.67) --
	( 85.21, 89.45) --
	( 85.46, 89.24) --
	( 85.72, 89.04) --
	( 85.97, 88.83) --
	( 86.22, 88.62) --
	( 86.48, 88.42) --
	( 86.73, 88.21) --
	( 86.98, 88.01) --
	( 87.24, 87.80) --
	( 87.49, 87.60) --
	( 87.74, 87.40) --
	( 88.00, 87.20) --
	( 88.25, 87.01) --
	( 88.51, 86.81) --
	( 88.76, 86.61) --
	( 89.01, 86.42) --
	( 89.27, 86.22) --
	( 89.52, 86.03) --
	( 89.77, 85.84) --
	( 90.03, 85.65) --
	( 90.28, 85.46) --
	( 90.53, 85.27) --
	( 90.79, 85.08) --
	( 91.04, 84.90) --
	( 91.30, 84.71) --
	( 91.55, 84.53) --
	( 91.80, 84.34) --
	( 92.06, 84.16) --
	( 92.31, 83.98) --
	( 92.56, 83.80) --
	( 92.82, 83.62) --
	( 93.07, 83.44) --
	( 93.32, 83.26) --
	( 93.58, 83.09) --
	( 93.83, 82.91) --
	( 94.09, 82.74) --
	( 94.34, 82.57) --
	( 94.59, 82.39) --
	( 94.85, 82.22) --
	( 95.10, 82.05) --
	( 95.35, 81.89) --
	( 95.61, 81.72) --
	( 95.86, 81.55) --
	( 96.12, 81.39) --
	( 96.37, 81.22) --
	( 96.62, 81.06) --
	( 96.88, 80.89) --
	( 97.13, 80.73) --
	( 97.38, 80.57) --
	( 97.64, 80.41) --
	( 97.89, 80.25) --
	( 98.14, 80.10) --
	( 98.40, 79.94) --
	( 98.65, 79.78) --
	( 98.91, 79.63) --
	( 99.16, 79.48) --
	( 99.41, 79.32) --
	( 99.67, 79.17) --
	( 99.92, 79.02) --
	(100.17, 78.87) --
	(100.43, 78.73) --
	(100.68, 78.58) --
	(100.93, 78.43) --
	(101.19, 78.29) --
	(101.44, 78.14) --
	(101.70, 78.00) --
	(101.95, 77.86) --
	(102.20, 77.71) --
	(102.46, 77.57) --
	(102.71, 77.43) --
	(102.96, 77.30) --
	(103.22, 77.16) --
	(103.47, 77.02) --
	(103.72, 76.89) --
	(103.98, 76.75) --
	(104.23, 76.62) --
	(104.49, 76.49) --
	(104.74, 76.35) --
	(104.99, 76.22) --
	(105.25, 76.09) --
	(105.50, 75.97) --
	(105.75, 75.84) --
	(106.01, 75.71) --
	(106.26, 75.59) --
	(106.51, 75.46) --
	(106.77, 75.34) --
	(107.02, 75.21) --
	(107.28, 75.09) --
	(107.53, 74.97) --
	(107.78, 74.85) --
	(108.04, 74.73) --
	(108.29, 74.61) --
	(108.54, 74.50) --
	(108.80, 74.38) --
	(109.05, 74.26) --
	(109.30, 74.15) --
	(109.56, 74.04) --
	(109.81, 73.92) --
	(110.07, 73.81) --
	(110.32, 73.70) --
	(110.57, 73.59) --
	(110.83, 73.48) --
	(111.08, 73.37) --
	(111.33, 73.27) --
	(111.59, 73.16) --
	(111.84, 73.05) --
	(112.09, 72.95) --
	(112.35, 72.85) --
	(112.60, 72.74) --
	(112.86, 72.64) --
	(113.11, 72.54) --
	(113.36, 72.44) --
	(113.62, 72.34) --
	(113.87, 72.24) --
	(114.12, 72.15) --
	(114.38, 72.05) --
	(114.63, 71.95) --
	(114.89, 71.86) --
	(115.14, 71.76) --
	(115.39, 71.67) --
	(115.65, 71.58) --
	(115.90, 71.49) --
	(116.15, 71.40) --
	(116.41, 71.31) --
	(116.66, 71.22) --
	(116.91, 71.13) --
	(117.17, 71.04) --
	(117.42, 70.96) --
	(117.68, 70.87) --
	(117.93, 70.79) --
	(118.18, 70.70) --
	(118.44, 70.62) --
	(118.69, 70.54) --
	(118.94, 70.45) --
	(119.20, 70.37) --
	(119.45, 70.29) --
	(119.70, 70.21) --
	(119.96, 70.13) --
	(120.21, 70.06) --
	(120.47, 69.98) --
	(120.72, 69.90) --
	(120.97, 69.83) --
	(121.23, 69.75) --
	(121.48, 69.68) --
	(121.73, 69.61) --
	(121.99, 69.53) --
	(122.24, 69.46) --
	(122.49, 69.39) --
	(122.75, 69.32) --
	(123.00, 69.25) --
	(123.26, 69.18) --
	(123.51, 69.11) --
	(123.76, 69.05) --
	(124.02, 68.98) --
	(124.27, 68.91) --
	(124.52, 68.85) --
	(124.78, 68.78) --
	(125.03, 68.72) --
	(125.28, 68.66) --
	(125.54, 68.59) --
	(125.79, 68.53) --
	(126.05, 68.47) --
	(126.30, 68.41) --
	(126.55, 68.35) --
	(126.81, 68.29) --
	(127.06, 68.23) --
	(127.31, 68.18) --
	(127.57, 68.12) --
	(127.82, 68.06) --
	(128.07, 68.01) --
	(128.33, 67.95) --
	(128.58, 67.90) --
	(128.84, 67.84) --
	(129.09, 67.79) --
	(129.34, 67.73) --
	(129.60, 67.68) --
	(129.85, 67.63) --
	(130.10, 67.58) --
	(130.36, 67.53) --
	(130.61, 67.48) --
	(130.87, 67.43) --
	(131.12, 67.38) --
	(131.37, 67.33) --
	(131.63, 67.29) --
	(131.88, 67.24) --
	(132.13, 67.19) --
	(132.39, 67.15) --
	(132.64, 67.10) --
	(132.89, 67.06) --
	(133.15, 67.01) --
	(133.40, 66.97) --
	(133.66, 66.92) --
	(133.91, 66.88) --
	(134.16, 66.84) --
	(134.42, 66.80) --
	(134.67, 66.76) --
	(134.92, 66.71) --
	(135.18, 66.67) --
	(135.43, 66.63) --
	(135.68, 66.60) --
	(135.94, 66.56) --
	(136.19, 66.52) --
	(136.45, 66.48) --
	(136.70, 66.44) --
	(136.95, 66.41) --
	(137.21, 66.37) --
	(137.46, 66.33) --
	(137.71, 66.30) --
	(137.97, 66.26) --
	(138.22, 66.23) --
	(138.47, 66.19) --
	(138.73, 66.16) --
	(138.98, 66.13) --
	(139.24, 66.09) --
	(139.49, 66.06) --
	(139.74, 66.03) --
	(140.00, 66.00) --
	(140.25, 65.97) --
	(140.50, 65.93) --
	(140.76, 65.90) --
	(141.01, 65.87) --
	(141.26, 65.84) --
	(141.52, 65.81) --
	(141.77, 65.78) --
	(142.03, 65.76) --
	(142.28, 65.73) --
	(142.53, 65.70) --
	(142.79, 65.67) --
	(143.04, 65.64) --
	(143.29, 65.62) --
	(143.55, 65.59) --
	(143.80, 65.56) --
	(144.05, 65.54) --
	(144.31, 65.51) --
	(144.56, 65.49) --
	(144.82, 65.46) --
	(145.07, 65.44) --
	(145.32, 65.41) --
	(145.58, 65.39) --
	(145.83, 65.37) --
	(146.08, 65.34) --
	(146.34, 65.32) --
	(146.59, 65.30) --
	(146.84, 65.27) --
	(147.10, 65.25) --
	(147.35, 65.23) --
	(147.61, 65.21) --
	(147.86, 65.19) --
	(148.11, 65.17) --
	(148.37, 65.15) --
	(148.62, 65.12) --
	(148.87, 65.10) --
	(149.13, 65.08) --
	(149.38, 65.06) --
	(149.64, 65.05) --
	(149.89, 65.03) --
	(150.14, 65.01) --
	(150.40, 64.99) --
	(150.65, 64.97) --
	(150.90, 64.95) --
	(151.16, 64.93) --
	(151.41, 64.92) --
	(151.66, 64.90) --
	(151.92, 64.88) --
	(152.17, 64.86) --
	(152.43, 64.85) --
	(152.68, 64.83) --
	(152.93, 64.81) --
	(153.19, 64.80) --
	(153.44, 64.78) --
	(153.69, 64.76) --
	(153.95, 64.75) --
	(154.20, 64.73) --
	(154.45, 64.72) --
	(154.71, 64.70) --
	(154.96, 64.69) --
	(155.22, 64.67) --
	(155.47, 64.66) --
	(155.72, 64.64) --
	(155.98, 64.63) --
	(156.23, 64.62) --
	(156.48, 64.60) --
	(156.74, 64.59) --
	(156.99, 64.58) --
	(157.24, 64.56) --
	(157.50, 64.55) --
	(157.75, 64.54) --
	(158.01, 64.52) --
	(158.26, 64.51) --
	(158.51, 64.50) --
	(158.77, 64.49) --
	(159.02, 64.47) --
	(159.27, 64.46) --
	(159.53, 64.45) --
	(159.78, 64.44) --
	(160.03, 64.43) --
	(160.29, 64.41) --
	(160.54, 64.40) --
	(160.80, 64.39) --
	(161.05, 64.38) --
	(161.30, 64.37) --
	(161.56, 64.36) --
	(161.81, 64.35) --
	(162.06, 64.34) --
	(162.32, 64.33) --
	(162.57, 64.32) --
	(162.82, 64.31) --
	(163.08, 64.30) --
	(163.33, 64.29) --
	(163.59, 64.28) --
	(163.84, 64.27) --
	(164.09, 64.26) --
	(164.35, 64.25) --
	(164.60, 64.24) --
	(164.85, 64.23) --
	(165.11, 64.22) --
	(165.36, 64.21) --
	(165.62, 64.20) --
	(165.87, 64.20) --
	(166.12, 64.19) --
	(166.38, 64.18) --
	(166.63, 64.17) --
	(166.88, 64.16) --
	(167.14, 64.15) --
	(167.39, 64.15) --
	(167.64, 64.14) --
	(167.90, 64.13) --
	(168.15, 64.12) --
	(168.41, 64.11) --
	(168.66, 64.11) --
	(168.91, 64.10) --
	(169.17, 64.09) --
	(169.42, 64.08) --
	(169.67, 64.08) --
	(169.93, 64.07) --
	(170.18, 64.06) --
	(170.43, 64.05) --
	(170.69, 64.05) --
	(170.94, 64.04) --
	(171.20, 64.03) --
	(171.45, 64.03) --
	(171.70, 64.02) --
	(171.96, 64.01) --
	(172.21, 64.01) --
	(172.46, 64.00) --
	(172.72, 63.99) --
	(172.97, 63.99) --
	(173.22, 63.98) --
	(173.48, 63.98) --
	(173.73, 63.97) --
	(173.99, 63.96) --
	(174.24, 63.96) --
	(174.49, 63.95) --
	(174.75, 63.95) --
	(175.00, 63.94) --
	(175.25, 63.94) --
	(175.51, 63.93) --
	(175.76, 63.92) --
	(176.01, 63.92) --
	(176.27, 63.91) --
	(176.52, 63.91) --
	(176.78, 63.90) --
	(177.03, 63.90) --
	(177.28, 63.89) --
	(177.54, 63.89) --
	(177.79, 63.88) --
	(178.04, 63.88) --
	(178.30, 63.87) --
	(178.55, 63.87) --
	(178.80, 63.86) --
	(179.06, 63.86) --
	(179.31, 63.85) --
	(179.57, 63.85) --
	(179.82, 63.84) --
	(180.07, 63.84) --
	(180.33, 63.83) --
	(180.58, 63.83) --
	(180.83, 63.82) --
	(181.09, 63.82) --
	(181.34, 63.82) --
	(181.59, 63.81) --
	(181.85, 63.81) --
	(182.10, 63.80) --
	(182.36, 63.80) --
	(182.61, 63.79) --
	(182.86, 63.79) --
	(183.12, 63.79) --
	(183.37, 63.78) --
	(183.62, 63.78) --
	(183.88, 63.77) --
	(184.13, 63.77) --
	(184.39, 63.77) --
	(184.64, 63.76) --
	(184.89, 63.76) --
	(185.15, 63.76) --
	(185.40, 63.75) --
	(185.65, 63.75) --
	(185.91, 63.74) --
	(186.16, 63.74) --
	(186.41, 63.74) --
	(186.67, 63.73) --
	(186.92, 63.73) --
	(187.18, 63.73) --
	(187.43, 63.72) --
	(187.68, 63.72) --
	(187.94, 63.72) --
	(188.19, 63.71) --
	(188.44, 63.71) --
	(188.70, 63.71) --
	(188.95, 63.70) --
	(189.20, 63.70) --
	(189.46, 63.70) --
	(189.71, 63.69) --
	(189.97, 63.69) --
	(190.22, 63.69) --
	(190.47, 63.68) --
	(190.73, 63.68) --
	(190.98, 63.68) --
	(191.23, 63.68) --
	(191.49, 63.67) --
	(191.74, 63.67) --
	(191.99, 63.67) --
	(192.25, 63.66) --
	(192.50, 63.66) --
	(192.76, 63.66) --
	(193.01, 63.66) --
	(193.26, 63.65) --
	(193.52, 63.65) --
	(193.77, 63.65) --
	(194.02, 63.64) --
	(194.28, 63.64) --
	(194.53, 63.64) --
	(194.78, 63.64) --
	(195.04, 63.63) --
	(195.29, 63.63) --
	(195.55, 63.63) --
	(195.80, 63.63) --
	(196.05, 63.62) --
	(196.31, 63.62) --
	(196.56, 63.62) --
	(196.81, 63.62) --
	(197.07, 63.61) --
	(197.32, 63.61) --
	(197.57, 63.61) --
	(197.83, 63.61) --
	(198.08, 63.61) --
	(198.34, 63.60) --
	(198.59, 63.60) --
	(198.84, 63.60) --
	(199.10, 63.60) --
	(199.35, 63.59) --
	(199.60, 63.59) --
	(199.86, 63.59) --
	(200.11, 63.59) --
	(200.37, 63.59) --
	(200.62, 63.58) --
	(200.87, 63.58) --
	(201.13, 63.58) --
	(201.38, 63.58) --
	(201.63, 63.58) --
	(201.89, 63.57) --
	(202.14, 63.57) --
	(202.39, 63.57) --
	(202.65, 63.57) --
	(202.90, 63.57) --
	(203.16, 63.56) --
	(203.41, 63.56) --
	(203.66, 63.56) --
	(203.92, 63.56) --
	(204.17, 63.56) --
	(204.42, 63.55) --
	(204.68, 63.55) --
	(204.93, 63.55) --
	(205.18, 63.55) --
	(205.44, 63.55) --
	(205.69, 63.55) --
	(205.95, 63.54) --
	(206.20, 63.54) --
	(206.45, 63.54) --
	(206.71, 63.54) --
	(206.96, 63.54) --
	(207.21, 63.54);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (238.49,173.45);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 55.28, 61.20) -- (207.21, 61.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 55.28, 61.20) -- ( 55.28, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 93.26, 61.20) -- ( 93.26, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (131.25, 61.20) -- (131.25, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (169.23, 61.20) -- (169.23, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (207.21, 61.20) -- (207.21, 55.20);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 55.28, 39.60) {-1.0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 93.26, 39.60) {-0.5};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (131.25, 39.60) {0.0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (169.23, 39.60) {0.5};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (207.21, 39.60) {1.0};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 63.25) -- ( 49.20,123.90);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 63.25) -- ( 43.20, 63.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 75.38) -- ( 43.20, 75.38);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 87.51) -- ( 43.20, 87.51);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 99.64) -- ( 43.20, 99.64);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,111.77) -- ( 43.20,111.77);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,123.90) -- ( 43.20,123.90);

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80, 63.25) {0};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80, 87.51) {40};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,111.77) {80};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 61.20) --
	(213.29, 61.20) --
	(213.29,124.25) --
	( 49.20,124.25) --
	cycle;
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (238.49,173.45);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (131.25, 28.60) {$\lambda$};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 10.80, 92.72) {$\overline{\mu}^{(2)}$};
\end{scope}
\begin{scope}
\path[clip] ( 49.20, 61.20) rectangle (213.29,124.25);
\definecolor{drawColor}{RGB}{211,211,211}

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] ( 49.20, 63.25) -- (213.29, 63.25);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] ( 49.20, 75.38) -- (213.29, 75.38);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] ( 49.20, 87.51) -- (213.29, 87.51);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] ( 49.20, 99.64) -- (213.29, 99.64);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] ( 49.20,111.77) -- (213.29,111.77);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] ( 49.20,123.90) -- (213.29,123.90);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] ( 55.28, 61.20) -- ( 55.28,124.25);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] ( 93.26, 61.20) -- ( 93.26,124.25);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (131.25, 61.20) -- (131.25,124.25);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (169.23, 61.20) -- (169.23,124.25);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (207.21, 61.20) -- (207.21,124.25);
\end{scope}
\end{tikzpicture}

